Length-Controlled AlpacaEval: A Simple Way to Debias Automatic Evaluators

LLM-based auto-annotators have become a key component of the LLM development process due to their cost-effectiveness and scalability compared to human-based evaluation. However, these auto-annotators can introduce biases that are hard to remove. Even simple, known confounders such as preference for longer outputs remain in existing automated evaluation metrics. We propose a simple regression analysis approach for controlling biases in auto-evaluations. As a real case study, we focus on reducing the length bias of AlpacaEval, a fast and affordable benchmark for instruction-tuned LLMs that uses LLMs to estimate response quality. Despite being highly correlated with human preferences, AlpacaEval is known to favor models that generate longer outputs. We introduce a length-controlled AlpacaEval that aims to answer the counterfactual question: "What would the preference be if the model's and baseline's output had the same length?" To achieve this, we first fit a generalized linear model to predict the biased auto-annotator's preferences based on the mediators we want to control for (length difference) and other relevant features. We then obtain length-controlled preferences by predicting preferences while conditioning the GLM with a zero difference in lengths. Length-controlling not only improves the robustness of the metric to manipulations in model verbosity, but we also find that it increases the Spearman correlation with LMSYS Chatbot Arena from 0.94 to 0.98.

==> text/desiderata.tex <==
\section{Desiderata}

Here are the main desired properties that we would like our length-controlled AlpacaEval to have.


\begin{enumerate}
\item[\textbf{D1}] \textbf{High correlation with humans} Rankings on the AlpacaEval leaderboard should have high Spearman (non-linear) correlation with human rankings from the Chatbot Arena. %We will consider the Spearman correlation with . %We use Spearman correlation as the Arena's ELO ratings are related to win rates via a non-linear logit so Pearson correlation do not make sense. 
The raw AlpacaEval has already a high correlation of \textbf{0.93} with the Arena despite the length bias because (1) humans are also length-biased; and (2) the considered models are realistic rather than adversarial ones that try to game the benchmark. 
%
\item[\textbf{D2}] \textbf{Low length gameability} One issue with a biased metric is that adversarial players may take advantage of it. 
For example, in AlpacaEval 2.0 the win rate for the baseline ($50\%$) increases to $64\%$ when prompted to ``give as much detail as possible'' and decreases to $23\%$ when prompted to ``be as concise as possible while still providing all the necessary information to answer the question''.
Such gaming won't be seen through correlations in realistic scenarios [D1],
so instead we will keep track of the relative variance of models prompted for verbosity/conciseness.
Note that humans may also be prone to length gameability, but it is important for a leaderboard like AlapcaEval that is typically interpreted as an evaluation of a model rather than a system (model+prompt). 
%
\item[\textbf{D3}] \textbf{Robustness to white-box adversarial attacks} One issue with simple corrections of biases such as length is that we introduce a direct approach to changing the win rate, which may then be gamed by postprocessing the model output. % (make more concise)
%s to increase the positive correction.
 %This is not an issue for the main use case of AlpacaEval: development, but we will keep track of it as it may be an issue for AlpacaEval's leaderboard. 
\end{enumerate}

In addition to the previous desiderata, which give metrics to optimize for. 
We would also like our length-controlled win rate to have a similar interpretation as standard win rate, be simple, be fast, be general, not require any reannotations, and be such that new models do not impact the metric of old models.

% \begin{itemize}
% \item \textbf{Similar interpretation as win rate} People are used to AlpacaEval's win rate, so we want to retain a similar interpretation. In particular, for any two models $m_1,m_2$ we would like 
% %\begin{equation}
% \begin{align*}
% \mathrm{win\_rate}(m1,m2) &\in [0,100]     \\
% \mathrm{win\_rate}(m1,m1) &= 50     \\
% \mathrm{win\_rate}(m1,m2) &= 100 - \mathrm{win\_rate}(m2,m1)
% \end{align*}
%
% \item \textbf{Independent post-processed corrections} We (1) do not want to have to rerun any annotations as that would be expensive for >100 models, and (2) we want to be able to correct each model independently so that metrics do not change when adding new models.
%
% \item[\textbf{D6}] \textbf{Generalilty} We would like a general procedure that we may use to control other biases down the line, e.g., biases for lists \tocite{} or bias towards model's that are similar from the autoannotator \tocite{}.
% \end{itemize}

Now that we know what we would like our length correction to look like, let's discuss the selected method for length-corrected AlpacaEval. 
In \tocref{} we then briefly discuss other corrections we considered.

